Deck of Cards method for Hierarchical, Robust and Stochastic Ordinal Regression

We consider the recently introduced application of the Deck of Cards Method (DCM) to ordinal regression proposing two extensions related to two main research trends in Multiple Criteria Decision Aiding, namely scaling and ordinal regression generalizations. On the one hand, procedures, different from DCM (e.g. AHP, BWM, MACBETH) to collect and elaborate Decision Maker's (DM's) preference information are considered to define an overall evaluation of reference alternatives. On the other hand, Robust Ordinal Regression and Stochastic Multicriteria Acceptability Analysis are used to offer the DM more detailed and realistic decision-support outcomes. More precisely, we take into account preference imprecision and indetermination through a set of admissible comprehensive evaluations of alternatives provided by the whole set of value functions compatible with DM's preference information rather than the univocal assessment obtained from a single value function. In addition, we also consider alternatives evaluated on a set of criteria hierarchically structured. The methodology we propose allows the DM to provide precise or imprecise information at different levels of the hierarchy of criteria. Like scaling procedures, the compatible value function we consider can be of a different nature, such as weighted sum, linear or general monotone value function, or Choquet integral. Consequently, the approach we propose is versatile and well-equipped to be adapted to DM's characteristics and requirements. The applicability of the proposed methodology is shown by a didactic example based on a large ongoing research project in which Italian regions are evaluated on criteria representing Circular Economy, Innovation-Driven Development and Smart Specialization Strategies.

==> BAR_par_ws_general.tex <==
\begin{table}
\caption{Imprecise Information - Parameters of the approximated barycenter}
%\setlength{\tabcolsep}{6pt}
%\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{ccccccccc}
\toprule
$w_{(\mathbf{1,1})}$&$w_{(\mathbf{1,2})}$&$w_{(\mathbf{1,3})}$&$w_{(\mathbf{2,1})}$&$w_{(\mathbf{2,2})}$&$w_{(\mathbf{2,3})}$&$w_{(\mathbf{3,1})}$&$w_{(\mathbf{3,2})}$&$w_{(\mathbf{3,3})}$\\
\midrule
%0.1314&0.1601&0.0039&0.4544&0.0495&0.0043&0.0244&0.1760&0.1590\\
0.1132&0.1413&0.0055&0.3909&0.0432&0.0045&0.0213&0.1470&0.1333\\
\bottomrule
\end{tabular}
\end{center}
\end{table}


==> BAR_ws_rank.tex <==
\begin{table}
\centering
\footnotesize
\caption{Imprecise Information - Ranking obtained using the approximation of the barycenter at the global and partial levels}
\label{}
\begin{subtable}{0.5\textwidth}
\centering
\caption{Global level - $g_{(\mathbf{0})}$}
\label{}
\begin{tabular}{cccc}
\toprule
Rank&Region&ID&$U(a_{j})$\\
\midrule
%1 & Lombardy & 4 & 0.79853 \\ 
%2 & Emilia-Romagna & 8 & 0.78864 \\ 
%3 & Piedmont & 1 & 0.74315 \\ 
%4 & Veneto & 6 & 0.74143 \\ 
%5 & Friuli-Venezia Giulia & 7 & 0.71873 \\ 
%6 & Lazio & 12 & 0.6795 \\ 
%7 & Trentino-South Tyrol & 5 & 0.65008 \\ 
%8 & Tuscany & 9 & 0.62914 \\ 
%9 & Marche & 11 & 0.59734 \\ 
%10 & Campania & 15 & 0.54965 \\ 
%11 & Umbria & 10 & 0.5328 \\ 
%12 & Basilicata & 17 & 0.52176 \\ 
%13 & Liguria & 3 & 0.52023 \\ 
%14 & Abruzzo & 13 & 0.50976 \\ 
%15 & Apulia & 16 & 0.46797 \\ 
%16 & Molise & 14 & 0.45539 \\ 
%17 & Sardinia & 20 & 0.4506 \\ 
%18 & Calabria & 18 & 0.44009 \\ 
%19 & Aosta Valley & 2 & 0.43615 \\ 
%20 & Sicily & 19 & 0.39159 \\ 
1& Lombardy &4&0.68507\\
2& Emilia-Romagna &8&0.67725\\
\textbf{3}&\textbf{ Piedmont }&\textbf{1}&\textbf{0.63784}\\
4& Veneto &6&0.63754\\
5& Friuli-Venezia Giulia &7&0.61808\\
\textbf{6}&\textbf{ Lazio }&\textbf{12}&\textbf{0.58197}\\
\textbf{7}&\textbf{ Trentino-South Tyrol }&\textbf{5}&\textbf{0.56066}\\
8& Tuscany &9&0.53991\\
9& Marche &11&0.51384\\
10& Campania &15&0.47194\\
\textbf{11}&\textbf{ Umbria }&\textbf{10}&\textbf{0.45911}\\
12& Basilicata &17&0.44823\\
13& Liguria &3&0.44756\\
\textbf{14}&\textbf{ Abruzzo }&\textbf{13}&\textbf{0.43893}\\
15& Apulia &16&0.40177\\
16& Molise &14&0.3919\\
17& Sardinia &20&0.38905\\
18& Calabria &18&0.37864\\
19& Aosta Valley &2&0.3774\\
20& Sicily &19&0.33549\\
\bottomrule
\end{tabular}
\end{subtable}% <---- don't forget this %
\begin{subtable}{0.5\textwidth}
\centering
\caption{Circular Economy $g_{(\mathbf{1})}$}
\label{}
\begin{tabular}{cccc}
\toprule
Rank&Region&ID&$U(a_{j})$\\
\midrule
%1 & Veneto & 6 & 0.18765 \\ 
%2 & Lombardy & 4 & 0.18233 \\ 
%3 & Trentino-South Tyrol & 5 & 0.18122 \\ 
%4 & Sardinia & 20 & 0.1785 \\ 
%5 & Basilicata & 17 & 0.17287 \\ 
%6 & Friuli-Venezia Giulia & 7 & 0.16892 \\ 
%7 & Piedmont & 1 & 0.16091 \\ 
%8 & Abruzzo & 13 & 0.16019 \\ 
%9 & Campania & 15 & 0.15774 \\ 
%10 & Umbria & 10 & 0.15405 \\ 
%11 & Marche & 11 & 0.14959 \\ 
%12 & Calabria & 18 & 0.14616 \\ 
%13 & Molise & 14 & 0.13405 \\ 
%14 & Aosta Valley & 2 & 0.13207 \\ 
%15 & Apulia & 16 & 0.12633 \\ 
%16 & Lazio & 12 & 0.12306 \\ 
%17 & Liguria & 3 & 0.12091 \\ 
%18 & Emilia-Romagna & 8 & 0.11641 \\ 
%19 & Tuscany & 9 & 0.11015 \\ 
%20 & Sicily & 19 & 0.090856 \\
1& Veneto &6&0.16497\\
2& Lombardy &4&0.16023\\
\textbf{3}&\textbf{ Trentino-South Tyrol }&\textbf{5}&\textbf{0.15999}\\
4& Sardinia &20&0.15675\\
5& Basilicata &17&0.15154\\
\textbf{6}&\textbf{ Friuli-Venezia Giulia }&\textbf{7}&\textbf{0.14851}\\
\textbf{7}&\textbf{ Piedmont }&\textbf{1}&\textbf{0.14144}\\
8& Abruzzo &13&0.14075\\
9& Campania &15&0.13838\\
10& Umbria &10&0.13564\\
\textbf{11}&\textbf{ Marche }&\textbf{11}&\textbf{0.13179}\\
12& Calabria &18&0.12818\\
13& Aosta Valley &2&0.11782\\
\textbf{14}&\textbf{ Molise }&\textbf{14}&\textbf{0.11746}\\
15& Apulia &16&0.11098\\
16& Lazio &12&0.10812\\
17& Liguria &3&0.10636\\
18& Emilia-Romagna &8&0.10318\\
19& Tuscany &9&0.097505\\
20& Sicily &19&0.079469\\
\bottomrule
\end{tabular}		
\end{subtable}
\begin{subtable}{0.5\textwidth}
\centering
\caption{Innovation-Driven Development $g_{(\mathbf{2})}$}
\label{}
\begin{tabular}{cccc}
\toprule 
Rank&Region&ID&$U(a_{j})$\\
\midrule
%1 & Emilia-Romagna & 8 & 0.43893 \\ 
%2 & Friuli-Venezia Giulia & 7 & 0.35153 \\ 
%3 & Piedmont & 1 & 0.34434 \\ 
%4 & Veneto & 6 & 0.33141 \\ 
%5 & Lombardy & 4 & 0.32937 \\ 
%6 & Trentino-South Tyrol & 5 & 0.31833 \\ 
%7 & Lazio & 12 & 0.31472 \\ 
%8 & Tuscany & 9 & 0.30493 \\ 
%9 & Marche & 11 & 0.27576 \\ 
%10 & Liguria & 3 & 0.26568 \\ 
%11 & Umbria & 10 & 0.23949 \\ 
%12 & Abruzzo & 13 & 0.20397 \\ 
%13 & Molise & 14 & 0.19782 \\ 
%14 & Campania & 15 & 0.19653 \\ 
%15 & Aosta Valley & 2 & 0.19579 \\ 
%16 & Apulia & 16 & 0.163 \\ 
%17 & Basilicata & 17 & 0.16238 \\ 
%18 & Sardinia & 20 & 0.16216 \\ 
%19 & Sicily & 19 & 0.14376 \\ 
%20 & Calabria & 18 & 0.1424 \\ 
1& Emilia-Romagna &8&0.37848\\
2& Friuli-Venezia Giulia &7&0.30325\\
\textbf{3}&\textbf{ Piedmont }&\textbf{1}&\textbf{0.297}\\
4& Veneto &6&0.28597\\
5& Lombardy &4&0.28441\\
\textbf{6}&\textbf{ Trentino-South Tyrol }&\textbf{5}&\textbf{0.27447}\\
\textbf{7}&\textbf{ Lazio }&\textbf{12}&\textbf{0.27139}\\
8& Tuscany &9&0.26303\\
9& Marche &11&0.2378\\
10& Liguria &3&0.22915\\
\textbf{11}&\textbf{ Umbria }&\textbf{10}&\textbf{0.20654}\\
12& Abruzzo &13&0.17597\\
13& Molise &14&0.1706\\
\textbf{14}&\textbf{ Campania }&\textbf{15}&\textbf{0.16966}\\
15& Aosta Valley &2&0.16893\\
16& Apulia &16&0.14076\\
17& Basilicata &17&0.14014\\
18& Sardinia &20&0.13996\\
19& Sicily &19&0.1242\\
20& Calabria &18&0.12297\\
\bottomrule
\end{tabular}		
\end{subtable}%
\begin{subtable}{0.5\textwidth}
\centering
\caption{Smart Specialization $g_{(\mathbf{3})}$}
\label{}
\begin{tabular}{cccc}
\toprule 
Rank&Region&ID&$U(a_{j})$\\
\midrule
%1 & Lombardy & 4 & 0.28682 \\ 
%2 & Lazio & 12 & 0.24171 \\ 
%3 & Piedmont & 1 & 0.23791 \\ 
%4 & Emilia-Romagna & 8 & 0.2333 \\ 
%5 & Veneto & 6 & 0.22238 \\ 
%6 & Tuscany & 9 & 0.21406 \\ 
%7 & Friuli-Venezia Giulia & 7 & 0.19828 \\ 
%8 & Campania & 15 & 0.19537 \\ 
%9 & Basilicata & 17 & 0.1865 \\ 
%10 & Apulia & 16 & 0.17865 \\ 
%11 & Marche & 11 & 0.17198 \\ 
%12 & Sicily & 19 & 0.15698 \\ 
%13 & Calabria & 18 & 0.15153 \\ 
%14 & Trentino-South Tyrol & 5 & 0.15054 \\ 
%15 & Abruzzo & 13 & 0.14559 \\ 
%16 & Umbria & 10 & 0.13925 \\ 
%17 & Liguria & 3 & 0.13364 \\ 
%18 & Molise & 14 & 0.12352 \\ 
%19 & Sardinia & 20 & 0.10994 \\ 
%20 & Aosta Valley & 2 & 0.10829 \\ 
1& Lombardy &4&0.24043\\
2& Lazio &12&0.20246\\
\textbf{3}&\textbf{ Piedmont }&\textbf{1}&\textbf{0.1994}\\
4& Emilia-Romagna &8&0.19559\\
5& Veneto &6&0.18659\\
\textbf{6}&\textbf{ Tuscany }&\textbf{9}&\textbf{0.17937}\\
\textbf{7}&\textbf{ Friuli-Venezia Giulia }&\textbf{7}&\textbf{0.16632}\\
8& Campania &15&0.1639\\
9& Basilicata &17&0.15654\\
10& Apulia &16&0.15002\\
\textbf{11}&\textbf{ Marche }&\textbf{11}&\textbf{0.14424}\\
12& Sicily &19&0.13182\\
13& Calabria &18&0.1275\\
\textbf{14}&\textbf{ Trentino-South Tyrol }&\textbf{5}&\textbf{0.12621}\\
15& Abruzzo &13&0.12221\\
16& Umbria &10&0.11693\\
17& Liguria &3&0.11205\\
18& Molise &14&0.10384\\
19& Sardinia &20&0.09234\\
20& Aosta Valley &2&0.090645\\
\bottomrule
\end{tabular}		
\end{subtable}
\end{table}

==> PWI_ws_general_L1.tex <==
\begin{table}
\footnotesize
\caption{Imprecise Information - Pairwise Winning Indices (PWIs) on Circular Economy}
\label{PWI_general_globally}
\setlength{\tabcolsep}{1pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|cccccccccccccccccccc}
\toprule
ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
%1&0&100&100&0&0&0&0&100&100&100&100&100&100&100&100&100&0&100&100&0\\
%2&0&0&100&0&0&0&0&100&100&0&0&100&0&22.68&0&100&0&0&100&0\\
%3&0&0&0&0&0&0&0&100&100&0&0&0&0&0&0&0&0&0&100&0\\
%4&100&100&100&0&82.2&0&100&100&100&100&100&100&100&100&100&100&100&100&100&100\\
%5&100&100&100&17.8&0&0&100&100&100&100&100&100&100&100&100&100&100&100&100&100\\
%6&100&100&100&100&100&0&100&100&100&100&100&100&100&100&100&100&100&100&100&100\\
%7&100&100&100&0&0&0&0&100&100&100&100&100&100&100&100&100&0&100&100&0\\
%8&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&100&0\\
%9&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0\\
%10&0&100&100&0&0&0&0&100&100&0&100&100&0&100&0&100&0&100&100&0\\
%11&0&100&100&0&0&0&0&100&100&0&0&100&0&100&0&100&0&100&100&0\\
%12&0&0&100&0&0&0&0&100&100&0&0&0&0&0&0&0&0&0&100&0\\
%13&0&100&100&0&0&0&0&100&100&100&100&100&0&100&100&100&0&100&100&0\\
%14&0&77.32&100&0&0&0&0&100&100&0&0&100&0&0&0&100&0&0&100&0\\
%15&0&100&100&0&0&0&0&100&100&100&100&100&0&100&0&100&0&100&100&0\\
%16&0&0&100&0&0&0&0&100&100&0&0&100&0&0&0&0&0&0&100&0\\
%17&100&100&100&0&0&0&100&100&100&100&100&100&100&100&100&100&0&100&100&0\\
%18&0&100&100&0&0&0&0&100&100&0&0&100&0&100&0&100&0&0&100&0\\
%19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%20&100&100&100&0&0&0&100&100&100&100&100&100&100&100&100&100&100&100&100&0\\
1&0&100&100&0&0&0&0&100&100&100&100&100&100&100&100&100&0&100&100&0\\
2&0&0&100&0&0&0&0&100&100&0&0&100&0&51.64&0&100&0&0&100&0\\
\textbf{3}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}\\
4&100&100&100&0&61.07&0&100&100&100&100&100&100&100&100&100&100&100&100&100&100\\
5&100&100&100&38.93&0&0&100&100&100&100&100&100&100&100&100&100&100&100&100&100\\
\textbf{6}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
\textbf{7}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}\\
8&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&100&0\\
9&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0\\
10&0&100&100&0&0&0&0&100&100&0&100&100&0&100&0&100&0&100&100&0\\
\textbf{11}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}\\
12&0&0&100&0&0&0&0&100&100&0&0&0&0&0&0&0&0&0&100&0\\
13&0&100&100&0&0&0&0&100&100&100&100&100&0&100&100&100&0&100&100&0\\
\textbf{14}&\textbf{0}&\textbf{48.36}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}\\
15&0&100&100&0&0&0&0&100&100&100&100&100&0&100&0&100&0&100&100&0\\
16&0&0&100&0&0&0&0&100&100&0&0&100&0&0&0&0&0&0&100&0\\
17&100&100&100&0&0&0&100&100&100&100&100&100&100&100&100&100&0&100&100&0\\
18&0&100&100&0&0&0&0&100&100&0&0&100&0&100&0&100&0&0&100&0\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
20&100&100&100&0&0&0&100&100&100&100&100&100&100&100&100&100&100&100&100&0\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> PWI_ws_general_L2.tex <==
\begin{table}
\footnotesize
\caption{Imprecise Information - Pairwise Winning Indices (PWIs) on Innovation-Driven Development}
\label{PWI_general_globally}
\setlength{\tabcolsep}{1pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|cccccccccccccccccccc}
\toprule
ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
%1&0&100&100&100&100&100&0&0&100&100&100&100&100&100&100&100&100&100&100&100\\
%2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0.53&100&100&100&100&100\\
%3&0&100&0&0&0&0&0&0&0&100&0&0&100&100&100&100&100&100&100&100\\
%4&0&100&100&0&100&0&0&0&100&100&100&100&100&100&100&100&100&100&100&100\\
%5&0&100&100&0&0&0&0&0&100&100&100&100&100&100&100&100&100&100&100&100\\
%6&0&100&100&100&100&0&0&0&100&100&100&100&100&100&100&100&100&100&100&100\\
%7&100&100&100&100&100&100&0&0&100&100&100&100&100&100&100&100&100&100&100&100\\
%8&100&100&100&100&100&100&100&0&100&100&100&100&100&100&100&100&100&100&100&100\\
%9&0&100&100&0&0&0&0&0&0&100&100&0&100&100&100&100&100&100&100&100\\
%10&0&100&0&0&0&0&0&0&0&0&0&0&100&100&100&100&100&100&100&100\\ 11&0&100&100&0&0&0&0&0&0&100&0&0&100&100&100&100&100&100&100&100\\
%12&0&100&100&0&0&0&0&0&100&100&100&0&100&100&100&100&100&100&100&100\\
%13&0&100&0&0&0&0&0&0&0&0&0&0&0&100&100&100&100&100&100&100\\
%14&0&100&0&0&0&0&0&0&0&0&0&0&0&0&92.06&100&100&100&100&100\\
%15&0&99.47&0&0&0&0&0&0&0&0&0&0&0&7.94&0&100&100&100&100&100\\
%16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&100&100&100\\
%17&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&100&100\\
%18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0\\
%20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&100&0\\
1&0&100&100&100&100&100&0&0&100&100&100&100&100&100&100&100&100&100&100&100\\
2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0.03&100&100&100&100&100\\
\textbf{3}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
4&0&100&100&0&100&0&0&0&100&100&100&100&100&100&100&100&100&100&100&100\\
5&0&100&100&0&0&0&0&0&100&100&100&100&100&100&100&100&100&100&100&100\\
\textbf{6}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
\textbf{7}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
8&100&100&100&100&100&100&100&0&100&100&100&100&100&100&100&100&100&100&100&100\\
9&0&100&100&0&0&0&0&0&0&100&100&0&100&100&100&100&100&100&100&100\\
10&0&100&0&0&0&0&0&0&0&0&0&0&100&100&100&100&100&100&100&100\\
\textbf{11}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
12&0&100&100&0&0&0&0&0&100&100&100&0&100&100&100&100&100&100&100&100\\
13&0&100&0&0&0&0&0&0&0&0&0&0&0&100&100&100&100&100&100&100\\
\textbf{14}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{89.41}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
15&0&99.97&0&0&0&0&0&0&0&0&0&0&0&10.59&0&100&100&100&100&100\\
16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&100&100&100\\
17&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&100&100\\
18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0\\
20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&100&0\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> PWI_ws_general_L3.tex <==
\begin{table}
\footnotesize
\caption{Imprecise Information - Pairwise Winning Indices (PWIs) on Smart Specialization}
\label{PWI_general_globally}
\setlength{\tabcolsep}{1pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|cccccccccccccccccccc}
\toprule
ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
%1&0&100&100&0&100&100&100&100&100&100&100&0&100&100&100&100&100&100&100&100\\
%2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&16.24\\
%3&0&100&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&100\\
%4&100&100&100&0&100&100&100&100&100&100&100&100&100&100&100&100&100&100&100&100\\
%5&0&100&100&0&0&0&0&0&0&100&0&0&100&100&0&0&0&37.46&0&100\\
%6&0&100&100&0&100&0&100&0&100&100&100&0&100&100&100&100&100&100&100&100\\
%7&0&100&100&0&100&0&0&0&0&100&100&0&100&100&100&100&100&100&100&100\\
%8&0&100&100&0&100&100&100&0&100&100&100&0&100&100&100&100&100&100&100&100\\
%9&0&100&100&0&100&0&100&0&0&100&100&0&100&100&100&100&100&100&100&100\\
%10&0&100&100&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&100\\
%11&0&100&100&0&100&0&0&0&0&100&0&0&100&100&0&0&0&100&100&100\\
%12&100&100&100&0&100&100&100&100&100&100&100&0&100&100&100&100&100&100&100&100\\
%13&0&100&100&0&0&0&0&0&0&100&0&0&0&100&0&0&0&0&0&100\\
%14&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100\\
%15&0&100&100&0&100&0&0&0&0&100&100&0&100&100&0&100&100&100&100&100\\
%16&0&100&100&0&100&0&0&0&0&100&100&0&100&100&0&0&0&100&100&100\\
%17&0&100&100&0&100&0&0&0&0&100&100&0&100&100&0&100&0&100&100&100\\
%18&0&100&100&0&62.54&0&0&0&0&100&0&0&100&100&0&0&0&0&0&100\\
%19&0&100&100&0&100&0&0&0&0&100&0&0&100&100&0&0&0&100&0&100\\
%20&0&83.76&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
1&0&100&100&0&100&100&100&100&100&100&100&0&100&100&100&100&100&100&100&100\\
2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&9.81\\
\textbf{3}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}\\
4&100&100&100&0&100&100&100&100&100&100&100&100&100&100&100&100&100&100&100&100\\
5&0&100&100&0&0&0&0&0&0&100&0&0&100&100&0&0&0&22.39&0&100\\
\textbf{6}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
\textbf{7}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
8&0&100&100&0&100&100&100&0&100&100&100&0&100&100&100&100&100&100&100&100\\
9&0&100&100&0&100&0&100&0&0&100&100&0&100&100&100&100&100&100&100&100\\
10&0&100&100&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&100\\
\textbf{11}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}\\
12&100&100&100&0&100&100&100&100&100&100&100&0&100&100&100&100&100&100&100&100\\
13&0&100&100&0&0&0&0&0&0&100&0&0&0&100&0&0&0&0&0&100\\
\textbf{14}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}\\
15&0&100&100&0&100&0&0&0&0&100&100&0&100&100&0&100&100&100&100&100\\
16&0&100&100&0&100&0&0&0&0&100&100&0&100&100&0&0&0&100&100&100\\
17&0&100&100&0&100&0&0&0&0&100&100&0&100&100&0&100&0&100&100&100\\
18&0&100&100&0&77.61&0&0&0&0&100&0&0&100&100&0&0&0&0&0&100\\
19&0&100&100&0&100&0&0&0&0&100&0&0&100&100&0&0&0&100&0&100\\
20&0&90.19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> PWI_ws_general_globally.tex <==
\begin{table}
\footnotesize
\caption{Imprecise Information - Pairwise Winning Indices (PWIs) on global level}
\label{PWI_general_globally}
\setlength{\tabcolsep}{1pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|cccccccccccccccccccc}
\toprule
ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
%1&0&100&100&0&100&87.62&100&0&100&100&100&100&100&100&100&100&100&100&100&100\\
%2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&8.29&100&0\\
%3&0&100&0&0&0&0&0&0&0&0&0&0&100&100&0&100&17.35&100&100&100\\
%4&100&100&100&0&100&100&100&100&100&100&100&100&100&100&100&100&100&100&100&100\\
%5&0&100&100&0&0&0&0&0&100&100&100&0&100&100&100&100&100&100&100&100\\
%6&12.38&100&100&0&100&0&100&0&100&100&100&100&100&100&100&100&100&100&100&100\\
%7&0&100&100&0&100&0&0&0&100&100&100&100&100&100&100&100&100&100&100&100\\
%8&100&100&100&0&100&100&100&0&100&100&100&100&100&100&100&100&100&100&100&100\\
%9&0&100&100&0&0&0&0&0&0&100&100&0&100&100&100&100&100&100&100&100\\
%10&0&100&100&0&0&0&0&0&0&0&0&0&100&100&0&100&100&100&100&100\\
%11&0&100&100&0&0&0&0&0&0&100&0&0&100&100&100&100&100&100&100&100\\
%12&0&100&100&0&100&0&0&0&100&100&100&0&100&100&100&100&100&100&100&100\\
%13&0&100&0&0&0&0&0&0&0&0&0&0&0&100&0&100&0&100&100&100\\
%14&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&100&100\\
%15&0&100&100&0&0&0&0&0&0&100&0&0&100&100&0&100&100&100&100&100\\
%16&0&100&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&100&100&100\\
%17&0&100&82.65&0&0&0&0&0&0&0&0&0&100&100&0&100&0&100&100&100\\
%18&0&91.71&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0\\
%19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%20&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&100&0\\
1&0&100&100&0&100&54.24&100&0&100&100&100&100&100&100&100&100&100&100&100&100\\
2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&34.82&100&0\\
\textbf{3}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{26.97}&\textbf{100}&\textbf{100}&\textbf{100}\\
4&100&100&100&0&100&100&100&100&100&100&100&100&100&100&100&100&100&100&100&100\\
5&0&100&100&0&0&0&0&0&100&100&100&0&100&100&100&100&100&100&100&100\\
\textbf{6}&\textbf{45.76}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
\textbf{7}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
8&100&100&100&0&100&100&100&0&100&100&100&100&100&100&100&100&100&100&100&100\\
9&0&100&100&0&0&0&0&0&0&100&100&0&100&100&100&100&100&100&100&100\\
10&0&100&100&0&0&0&0&0&0&0&0&0&100&100&0&100&100&100&100&100\\
\textbf{11}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}&\textbf{100}\\
12&0&100&100&0&100&0&0&0&100&100&100&0&100&100&100&100&100&100&100&100\\
13&0&100&0&0&0&0&0&0&0&0&0&0&0&100&0&100&0&100&100&100\\
\textbf{14}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{100}&\textbf{91.13}\\
15&0&100&100&0&0&0&0&0&0&100&0&0&100&100&0&100&100&100&100&100\\
16&0&100&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&100&100&100\\
17&0&100&73.03&0&0&0&0&0&0&0&0&0&100&100&0&100&0&100&100&100\\
18&0&65.18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
20&0&100&0&0&0&0&0&0&0&0&0&0&0&8.87&0&0&0&100&100&0\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> RAI_ws_general_L1.tex <==
\begin{table}
\footnotesize
\caption{Imprecise information - Rank Acceptability Indices (RAIs) on Circular Economy}
\label{RAI_general_g1}
\setlength{\tabcolsep}{1pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{>{\centering}m{0.06\textwidth}|cccccccccccccccccccc}
\toprule
Rank ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
%1&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%2&0&0&0&0&0&0&0&0&0&0&0&0&22.68&77.32&0&0&0&0&0&0\\
%3&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0\\
%4&0&82.2&17.8&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%5&0&17.8&82.2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%6&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%7&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%8&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0\\
%9&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0\\
%10&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0\\
%11&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0\\
%12&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0\\
%13&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0\\
%14&0&0&0&0&0&0&0&0&0&0&0&0&77.32&22.68&0&0&0&0&0&0\\
%15&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0\\
%16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0\\
%17&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%18&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0\\
%19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100\\
%20&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
1&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0\\
2&0&0&0&0&0&0&0&0&0&0&0&0&51.64&48.36&0&0&0&0&0&0\\
\textbf{3}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}\\
4&0&61.07&38.93&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
5&0&38.93&61.07&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
\textbf{6}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
\textbf{7}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
8&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0\\
9&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0\\
10&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0\\
\textbf{11}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
12&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0\\
13&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0\\
\textbf{14}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{48.36}&\textbf{51.64}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
15&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0\\
16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0\\
17&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
18&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100\\
20&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> RAI_ws_general_L2.tex <==
\begin{table}
\footnotesize
\caption{Imprecise Information - Rank Acceptability Indices (RAIs) on Innovation-Driven Development}
\label{RAI_general_g2}
\setlength{\tabcolsep}{1pt} \renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{>{\centering}m{0.06\textwidth}|cccccccccccccccccccc}
\toprule
Rank ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
%1&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%2&0&0&0&0&0&0&0&0&0&0&0&0&0&0.53&99.47&0&0&0&0&0\\
%3&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0\\
%4&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%5&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%6&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%7&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%8&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%9&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0\\
%10&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0\\
%11&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0\\
%12&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%13&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0\\
%14&0&0&0&0&0&0&0&0&0&0&0&0&92.06&7.94&0&0&0&0&0&0\\
%15&0&0&0&0&0&0&0&0&0&0&0&0&7.94&91.52&0.53&0&0&0&0&0\\
%16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0\\
%17&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0\\
%18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100\\
%19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0\\
%20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0\\
1&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
2&0&0&0&0&0&0&0&0&0&0&0&0&0&0.03&99.97&0&0&0&0&0\\
\textbf{3}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
4&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
5&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
\textbf{6}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
\textbf{7}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
8&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
9&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0\\
10&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0\\
\textbf{11}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
12&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0\\
13&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0\\
\textbf{14}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{89.41}&\textbf{10.59}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
15&0&0&0&0&0&0&0&0&0&0&0&0&10.59&89.38&0.03&0&0&0&0&0\\
16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0\\
17&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0\\
18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0\\
20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> RAI_ws_general_L3.tex <==
\begin{table}
\footnotesize
\caption{Imprecise Information - Rank Acceptability Indices (RAIs) on Smart Specialization}
\label{RAI_general_g3}
\setlength{\tabcolsep}{1pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{>{\centering}m{0.06\textwidth}|cccccccccccccccccccc}
\toprule
Rank ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
%1&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&16.24&83.76\\
%3&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0\\
%4&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%5&0&0&0&0&0&0&0&0&0&0&0&0&37.46&62.54&0&0&0&0&0&0\\
%6&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%7&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%8&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%9&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%10&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0\\
%11&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0\\
%12&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%13&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0\\
%14&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0\\
%15&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0\\
%16&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0\\
%17&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0\\
%18&0&0&0&0&0&0&0&0&0&0&0&0&62.54&37.46&0&0&0&0&0&0\\
%19&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0\\
%20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&83.76&16.24\\
1&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&9.81&90.19\\
\textbf{3}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}\\
4&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
5&0&0&0&0&0&0&0&0&0&0&0&0&22.39&77.61&0&0&0&0&0&0\\
\textbf{6}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
\textbf{7}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
8&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
9&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
10&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0\\
\textbf{11}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
12&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
13&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0\\
\textbf{14}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}\\
15&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0\\
16&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0\\
17&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0\\
18&0&0&0&0&0&0&0&0&0&0&0&0&77.61&22.39&0&0&0&0&0&0\\
19&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0\\
20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&90.19&9.81\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> RAI_ws_general_globally.tex <==
\begin{table}
\footnotesize
\caption{Imprecise Information - Rank Acceptability Indices (RAIs) on global level}
\label{RAI_general_globally}
\setlength{\tabcolsep}{1pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{>{\centering}m{0.06\textwidth}|cccccccccccccccccccc}
\toprule
Rank ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
%1&0&0&87.62&12.38&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&8.29&91.71&0\\
%3&0&0&0&0&0&0&0&0&0&0&0&17.35&82.65&0&0&0&0&0&0&0\\
%4&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%5&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%6&0&0&12.38&87.62&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%7&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%8&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%9&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0\\
%10&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0\\
%11&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0\\
%12&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
%13&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0\\
%14&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0\\
%15&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0\\
%16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0\\
%17&0&0&0&0&0&0&0&0&0&0&0&82.65&17.35&0&0&0&0&0&0&0\\
%18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&91.71&8.29&0\\
%19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100\\
%20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0\\
1&0&0&54.24&45.76&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
2&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&34.82&65.18&0\\
\textbf{3}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{26.97}&\textbf{73.03}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
4&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
5&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0\\
\textbf{6}&\textbf{0}&\textbf{0}&\textbf{45.76}&\textbf{54.24}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
\textbf{7}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
8&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
9&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0\\
10&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0\\
\textbf{11}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{100}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}\\
12&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
13&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0\\
\textbf{14}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{91.13}&\textbf{8.87}&\textbf{0}&\textbf{0}&\textbf{0}\\
15&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0&0&0&0&0&0\\
16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100&0&0&0&0&0\\
17&0&0&0&0&0&0&0&0&0&0&0&73.03&26.97&0&0&0&0&0&0&0\\
18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&65.18&34.82&0\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&100\\
20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&8.87&91.13&0&0&0\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> necc_ws_general.tex <==
\begin{table}[h!]
\footnotesize
\caption{Imprecise Information - Necessary preference relation between regions on global level}
\label{NECgeneral}
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|rrrrrrrrrrrrrrrrrrrr}
\toprule
ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
%1&1&1&1&0&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
%2&0&1&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0\\
%3&0&0&1&0&0&0&0&0&0&0&0&0&0&1&0&1&0&1&1&0\\
%4&1&1&1&1&0&0&1&0&1&1&1&1&1&1&1&1&1&1&1&1\\
%5&0&1&1&0&1&0&0&0&0&1&1&0&1&1&1&1&1&1&1&1\\
%6&0&1&1&0&0&1&1&0&1&1&1&1&1&1&1&1&1&1&1&1\\
%7&0&1&1&0&0&0&1&0&1&1&1&1&1&1&1&1&1&1&1&1\\
%8&0&1&1&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1&1\\
%9&0&0&0&0&0&0&0&0&1&0&0&0&0&1&0&1&0&1&1&0\\
%10&0&0&1&0&0&0&0&0&0&1&0&0&1&1&0&1&0&1&1&0\\
%11&0&0&1&0&0&0&0&0&0&1&1&0&1&1&1&1&1&1&1&0\\
%12&0&0&1&0&0&0&0&0&1&0&0&1&0&1&0&1&0&1&1&0\\
%13&0&0&0&0&0&0&0&0&0&0&0&0&1&1&0&1&0&1&1&0\\
%14&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&0&0&1&1&0\\
%15&0&0&1&0&0&0&0&0&0&0&0&0&0&1&1&1&0&1&1&0\\
%16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&0&1&0\\
%17&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&1&1&1&1&0\\
%18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&0\\
%19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0\\
%20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1\\
1&1&1&1&0&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
2&0&1&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0\\
\textbf{3}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}\\
4&1&1&1&1&0&0&1&0&1&1&1&1&1&1&1&1&1&1&1&1\\
5&0&1&1&0&1&0&0&0&0&1&1&0&1&1&1&1&1&1&1&1\\
\textbf{6}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
\textbf{7}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
8&0&1&1&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1&1\\
9&0&0&0&0&0&0&0&0&1&0&0&0&0&1&0&1&0&1&1&0\\
10&0&0&1&0&0&0&0&0&0&1&0&0&1&1&0&1&0&1&1&0\\
\textbf{11}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}\\
12&0&0&1&0&0&0&0&0&1&0&0&1&0&1&0&1&0&1&1&0\\
13&0&0&0&0&0&0&0&0&0&0&0&0&1&1&0&1&0&1&1&0\\
\textbf{14}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}\\
15&0&0&1&0&0&0&0&0&0&0&0&0&0&1&1&1&0&1&1&0\\
16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&0&1&0\\
17&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&1&1&1&1&0\\
18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&0\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0\\
20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> necc_ws_l1.tex <==
\begin{table}[h!]
\footnotesize
\caption{Imprecise Information - Necessary preference relation between regions on Circular Economy}
\label{NECgeneral}
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|rrrrrrrrrrrrrrrrrrrr}
\toprule
ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
1&1&0&1&0&0&0&0&1&1&1&1&1&1&1&1&1&0&1&1&0\\
2&0&1&1&0&0&0&0&1&1&0&0&1&0&0&0&1&0&0&1&0\\
\textbf{3}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}\\
4&1&0&1&1&0&0&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
5&1&1&1&0&1&0&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{6}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
\textbf{7}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}\\
8&0&0&0&0&0&0&0&1&1&0&0&0&0&0&0&0&0&0&1&0\\
9&0&0&0&0&0&0&0&0&1&0&0&0&0&0&0&0&0&0&1&0\\
10&0&0&1&0&0&0&0&1&1&1&1&1&0&1&0&1&0&1&1&0\\
\textbf{11}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}\\
12&0&0&1&0&0&0&0&0&0&0&0&1&0&0&0&0&0&0&1&0\\
13&0&0&1&0&0&0&0&1&1&1&1&1&1&1&1&1&0&1&1&0\\
\textbf{14}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}\\
15&0&0&1&0&0&0&0&1&1&0&0&1&0&1&1&1&0&1&1&0\\
16&0&0&1&0&0&0&0&0&1&0&0&1&0&0&0&1&0&0&1&0\\
17&1&0&1&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1&0\\
18&0&0&1&0&0&0&0&1&1&0&0&1&0&1&0&1&0&1&1&0\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0\\
20&1&0&1&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> necc_ws_l2.tex <==
\begin{table}[h!]
\footnotesize
\caption{Imprecise Information - Necessary preference relation between regions on Innovation-Driven Development}
\label{NECgeneral}
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|rrrrrrrrrrrrrrrrrrrr}
\toprule
ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
1&1&1&1&1&1&1&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
2&0&1&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&1&1&1\\
\textbf{3}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
4&0&1&1&1&1&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
5&0&1&1&0&1&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{6}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
\textbf{7}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
8&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
9&0&1&1&0&0&0&0&0&1&1&1&0&1&1&1&1&1&1&1&1\\
10&0&1&0&0&0&0&0&0&0&1&0&0&1&1&1&1&1&1&1&1\\
\textbf{11}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
12&0&1&1&0&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
13&0&1&0&0&0&0&0&0&0&0&0&0&1&1&1&1&1&1&1&1\\
\textbf{14}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
15&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&1&1&1&1\\
16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&1&1&1\\
17&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&1&1\\
18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&0\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&0\\
20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&1\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> necc_ws_l3.tex <==
\begin{table}[h!]
\footnotesize
\caption{Imprecise Information - Necessary preference relation between regions on Smart Specialization}
\label{NECgeneral}
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|rrrrrrrrrrrrrrrrrrrr}
\toprule
ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
1&1&1&1&0&1&1&1&1&1&1&1&0&1&1&1&1&1&1&1&1\\
2&0&1&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\
\textbf{3}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}\\
4&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
5&0&1&1&0&1&0&0&0&0&1&0&0&1&1&0&0&0&0&0&1\\
\textbf{6}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
\textbf{7}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
8&0&1&1&0&1&1&1&1&1&1&1&0&1&1&1&1&1&1&1&1\\
9&0&1&1&0&1&0&1&0&1&1&1&0&1&1&1&1&1&1&1&1\\
10&0&1&0&0&0&0&0&0&0&1&0&0&0&1&0&0&0&0&0&1\\
\textbf{11}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}\\
12&1&1&1&0&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
13&0&1&1&0&0&0&0&0&0&1&0&0&1&1&0&0&0&0&0&1\\
\textbf{14}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}\\
15&0&1&1&0&1&0&0&0&0&1&1&0&1&1&1&1&0&1&1&1\\
16&0&1&1&0&1&0&0&0&0&1&0&0&1&1&0&1&0&1&1&1\\
17&0&1&1&0&1&0&0&0&0&1&1&0&1&1&0&1&1&1&1&1\\
18&0&1&1&0&0&0&0&0&0&1&0&0&0&1&0&0&0&1&0&1\\
19&0&1&1&0&0&0&0&0&0&1&0&0&1&1&0&0&0&1&1&1\\
20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> poss_ws_general.tex <==
\begin{table}[h!]
\footnotesize
\caption{Imprecise Information - Possible preference relation between regions on global level}
\label{POSgeneral}
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|rrrrrrrrrrrrrrrrrrrr}
\toprule ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
%1&1&1&1&0&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
%2&0&1&1&0&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
%3&0&1&1&0&0&0&0&0&1&0&0&0&1&1&0&1&1&1&1&1\\
%4&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
%5&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
%6&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
%7&1&1&1&0&1&0&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
%8&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
%9&0&1&1&0&1&0&0&0&1&1&1&0&1&1&1&1&1&1&1&1\\
%10&0&1&1&0&0&0&0&0&1&1&0&1&1&1&1&1&1&1&1&1\\
%11&0&1&1&0&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
%12&0&1&1&0&1&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
%13&0&1&1&0&0&0&0&0&1&0&0&1&1&1&1&1&1&1&1&1\\
%14&0&1&0&0&0&0&0&0&0&0&0&0&0&1&0&1&0&1&1&1\\
%15&0&1&1&0&0&0&0&0&1&1&0&1&1&1&1&1&1&1&1&1\\
%16&0&1&0&0&0&0&0&0&0&0&0&0&0&1&0&1&0&1&1&1\\
%17&0&1&1&0&0&0&0&0&1&1&0&1&1&1&1&1&1&1&1&1\\
%18&0&1&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&1&1&1\\
%19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0\\
%20&0&1&1&0&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
1&1&1&1&0&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
2&0&1&1&0&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{3}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
4&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
5&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{6}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
\textbf{7}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
8&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
9&0&1&1&0&1&0&0&0&1&1&1&0&1&1&1&1&1&1&1&1\\
10&0&1&1&0&0&0&0&0&1&1&0&1&1&1&1&1&1&1&1&1\\
\textbf{11}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
12&0&1&1&0&1&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
13&0&1&1&0&0&0&0&0&1&0&0&1&1&1&1&1&1&1&1&1\\
\textbf{14}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}\\
15&0&1&1&0&0&0&0&0&1&1&0&1&1&1&1&1&1&1&1&1\\
16&0&1&0&0&0&0&0&0&0&0&0&0&0&1&0&1&0&1&1&1\\
17&0&1&1&0&0&0&0&0&1&1&0&1&1&1&1&1&1&1&1&1\\
18&0&1&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&1&1&1\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0\\
20&0&1&1&0&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> poss_ws_l1.tex <==
\begin{table}[h!]
\footnotesize
\caption{Imprecise Information - Possible preference relation between regions on Circular Economy}
\label{POSgeneral}
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|rrrrrrrrrrrrrrrrrrrr}
\toprule ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
1&1&1&1&0&0&0&0&1&1&1&1&1&1&1&1&1&0&1&1&0\\
2&1&1&1&1&0&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{3}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}\\
4&1&1&1&1&1&0&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
5&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{6}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
\textbf{7}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}\\
8&0&0&1&0&0&0&0&1&1&0&0&1&0&1&0&1&0&0&1&0\\
9&0&0&1&0&0&0&0&0&1&0&0&1&0&0&0&0&0&0&1&0\\
10&0&1&1&0&0&0&0&1&1&1&1&1&0&1&1&1&0&1&1&0\\
\textbf{11}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}\\
12&0&0&1&0&0&0&0&1&1&0&0&1&0&0&0&0&0&0&1&0\\
13&0&1&1&0&0&0&0&1&1&1&1&1&1&1&1&1&0&1&1&0\\
\textbf{14}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}\\
15&0&1&1&0&0&0&0&1&1&1&1&1&0&1&1&1&0&1&1&0\\
16&0&0&1&0&0&0&0&1&1&0&0&1&0&0&0&1&0&0&1&0\\
17&1&1&1&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1&1&0\\
18&0&1&1&0&0&0&0&1&1&0&0&1&0&1&0&1&0&1&1&0\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0\\
20&1&1&1&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> poss_ws_l2.tex <==
\begin{table}[h!]
\footnotesize
\caption{Imprecise Information - Possible preference relation between regions on Innovation-Driven Development}
\label{POSgeneral}
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|rrrrrrrrrrrrrrrrrrrr}
\toprule ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
1&1&1&1&1&1&1&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
2&0&1&0&0&0&0&0&0&0&0&0&0&0&1&1&1&1&1&1&1\\
\textbf{3}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
4&0&1&1&1&1&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
5&0&1&1&0&1&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{6}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
\textbf{7}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
8&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
9&0&1&1&0&0&0&0&0&1&1&1&0&1&1&1&1&1&1&1&1\\
10&0&1&0&0&0&0&0&0&0&1&0&0&1&1&1&1&1&1&1&1\\
\textbf{11}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
12&0&1&1&0&0&0&0&0&1&1&1&1&1&1&1&1&1&1&1&1\\
13&0&1&0&0&0&0&0&0&0&0&0&0&1&1&1&1&1&1&1&1\\
\textbf{14}&\textbf{0}&\textbf{1}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{0}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
15&0&1&0&0&0&0&0&0&0&0&0&0&0&1&1&1&1&1&1&1\\
16&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&1&1&1\\
17&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&1&1\\
18&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&0&0\\
19&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&0\\
20&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&1&1&1\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

==> poss_ws_l3.tex <==
\begin{table}[h!]
\footnotesize
\caption{Imprecise Information - Possible preference relation between regions on Smart Specialization}
\label{POSgeneral}
\setlength{\tabcolsep}{6pt}
\renewcommand\arraystretch{1}
\begin{center}
\begin{tabular}{c|rrrrrrrrrrrrrrrrrrrr}
\toprule ID&1&2&3&4&5&6&7&8&9&10&11&12&13&14&15&16&17&18&19&20\\
\midrule
1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
2&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{3}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
4&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
5&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{6}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
\textbf{7}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
8&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
9&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
10&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{11}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
12&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
13&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\textbf{14}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}&\textbf{1}\\
15&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
16&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
17&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
18&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
19&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
20&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1&1\\
\bottomrule
\end{tabular}
\end{center}
\end{table}
